Extending local features with contextual information in graph kernels

Graph kernels are usually defined in terms of simpler kernels over local substructures of the original graphs. Different kernels consider different types of substructures. However, in some cases they have similar predictive performances, probably because the substructures can be interpreted as approximations of the subgraphs they induce. In this paper, we propose to associate to each feature a piece of information about the context in which the feature appears in the graph. A substructure appearing in two different graphs will match only if it appears with the same context in both graphs. We propose a kernel based on this idea that considers trees as substructures, and where the contexts are features too. The kernel is inspired from the framework in [6], even if it is not part of it. We give an efficient algorithm for computing the kernel and show promising results on real-world graph classification datasets.

==> ICONIP15(CameraReady)/experiments.tex <==
\section{Experimental results}
We measured the predictive performance of TCK and other state-of-the-art kernels on the following real-world datasets: AIDS, CAS, CPDB, GDD and NCI1. Each dataset represents a binary classification problem
%. All the datasets are 
and is composed by labeled graphs with no self-loops. The AIDS, CAS, CPDB and NCI1 datasets are collections of chemical compounds represented as graphs, with nodes labeled according to the atom type and edges that represent the bonds. The GDD dataset is composed by proteins represented as graphs, where the nodes 
%of the graphs 
represent amino acids and two nodes in a graph are connected by an edge if they are less than $6$\,\AA\, apart. The largest datasets are CAS and NCI1 with more than 4000 graphs, and the smallest is CPDB with 684 instances.\\
Since we cannot know in advance whether the sparsity is beneficial for a particular task, we choose to test two versions of the proposed kernel. 
The first version ($TCK$) considers only contextualized features, while the second version ($TCK+ODDK$) combines $TCK$ with the base (non-contextualized) kernel, $ODDK$ in our case.
Note that $TCK+ODDK$ can be computed with a slight modification of Algorithm~\ref{alg:decomposeexpl}, thus the computational complexities of the two versions of the proposed kernels are the same.
%
\noindent We compare the proposed kernels with the NSPDK kernel~\cite{Costa2010}, the Fast Subtree Kernel (FS)~\cite{ShervashidzeSLMB11}, and the original version of the ODDK based on the subtree kernel~\cite{Dasan2012}. To assess the predictive performances of the different kernels, we used a \textit{nested} 10-fold cross validation: within each of the 10 folds, another 10-fold cross validation is performed over the corresponding training set in order to select the best parameters for the current fold. Thus, the parameters are optimized on the training dataset only.
The whole process has been repeated 10 times using different random data splits.
% and we report in Table \ref{Tab:nested} the averaged results with the corresponding standard deviations of the standard accuracy measure.
The parameter space for both versions of $TCK$ and $ODDK$ was restricted to the following values: $h=\{1,2,\dots,10\}$ and %$\lambda=\{0.1,0.5,0.8,0.9,1.0,1.1,1.2,1.3,1.4,1.5,1.8\}$. 
$\lambda=\{0.1,0.5,0.8,0.9,\ldots,1.5,1.8\}$.
%The parameters of the $ODDK$ ranged over $\lambda=\{0.1,0.2,\dots,2.0\}$ and $h=\{1,2,\dots,10\}$. 
The parameter $h$ of the FS kernel were restricted to $h=\{1,2,\dots,10\}$ and for the NSPDK the values $h=\{1,2,\dots,8\}$ and $d=\{1,2,\dots,7\}$ were considered.
The SVM solver had the $C$ parameter ranging in $C=\{10^{-4},10^{-3},\ldots,10^{3}\}$.
\begin{table}[t]
    \caption{Accuracy results of the proposed kernels and the considered baselines, in nested 10-fold cross validation.}\label{Tab:nested}
\centering
    \begin{tabular}{ | l | c | c | c | c | c |}
    \hline
        \textit{Kernel/dataset} & {CAS} & {GDD} & {NCI1} & {AIDS} & {CPDB}  \\ \hline
    $NSPDK$ & $83.6_{\pm0.34}$ & 74.09$_{\pm0.91}$ &  $83.46_{\pm0.46}$ & $82.71_{\pm0.66}$ & $76.99_{\pm1.15}$  \\
    $WL$ & $83.33_{\pm0.37}$ & $75.29_{\pm1.33}$ &  $84.41_{\pm0.49}$ & $82.02_{\pm0.4}$ & $76.36_{\pm1.4}$  \\
    $ODDK$ & $83.53_{\pm0.21}$ & $76.99_{\pm0.36}$ &  $85.31_{\pm0.26}$ & \textbf{82.99}$_{\pm0.50}$ & $78.44_{\pm0.76}$ \\ \hline
    $TCK$ & $83.53_{\pm0.32}$ & \textbf{79.35}$_{\pm0.45}$ & \textbf{85.78}$_{\pm0.22}$ & $82.88_{\pm0.39}$ & $76.96_{\pm0.96}$ \\
    $TCK+ODDK$ & \textbf{83.94}$_{\pm0.26}$ & $78.03_{\pm0.56}$ & $85.48_{\pm0.182}$ & $82.97_{\pm0.5}$ & \textbf{78.89}$_{\pm0.98}$ \\
 \hline
    %$ODDWCK_{sep}$ & \makecell{$0.8374_{\pm0.018}$ \\ \footnotesize{$h=5,\lambda=1.3, C=10$}} & \makecell{$0.7963_{\pm0.048}$ \\ \footnotesize{$h=2,\lambda=0.1, C=10$}} & \makecell{$0.8148_{\pm0.039}$ \\ \footnotesize{$h=6,\lambda=1.2, C=10$}} & \makecell{$0.8104_{\pm0.0396}$ \\ \footnotesize{$h=4,\lambda=1.5, C=1$}} & \makecell{$0.8026_{\pm0.035}$ \\ \footnotesize{$h=4,\lambda=1.4, C=100$}} & \makecell{$0.8881_{\pm0.0536}$ \\ \footnotesize{$h=3,\lambda=0.1, C=100$}}\\ \hline
    \end{tabular}
    % (the parameters are optimized on the training dataset only).

\end{table}
\begin{figure}[t]
\centering
  \includegraphics[width=0.72\textwidth]{Tempi/times_journal_CAS}
  \caption{Copmuptational time (in seconds) required for the Gram matrix computation of the considered kernel, with different parameters.\label{fig:times}}
\end{figure}
Table~\ref{Tab:nested} reports the averaged accuracy results of our experiments with the corresponding standard deviations.
At a first glance, it is clear that in almost all the considered datasets, one of the two proposed kernels is the better performing among all the considered kernels, with the only exception of the AIDS dataset.
Looking at the results in more detail, in two datasets (GDD, NCI1) both versions of $TCK$ perform better than the others. If we consider the CAS dataset, the performance of the worst of the proposed kernels is comparable with the better kernel among the baselines (NSPDK). In the CPDB dataset the worst of the proposed kernels
 is worse than the best kernel among the baselines (ODDK), but it 
 is still competitive, such as in AIDS dataset, where the proposed kernels are very close to the best one.
%Moreover, looking at the performances of the proposed kernels with respect to the ODDK kernel (the base kernel for $TCK$), we can see that the introduction of contexts can greatly improve the predictive performance of the kernel.
% \begin{figure}[t]
% \centering
%   \includegraphics[width=0.70\textwidth]{Tempi/times_journal_CAS}
%   \caption{Copmuptational time (in seconds) required for the Gram matrix computation of the considered kernel, with different parameters.\label{fig:times}}
% \end{figure}
\noindent Let us finally anlyze the computational requirements of our proposed kernel. Figure~\ref{fig:times} reports the computational times required for the Gram matrix computation of the kernels considered in this section on the CAS dataset.
The execution times of the proposed kernel are very close to the ones of the original kernel. The situation is similar for other datasets, and thus the corresponding plots are omitted.
% \begin{figure}[t]
% \centering
%   \includegraphics[width=0.70\textwidth]{Tempi/times_journal_CAS}
%   \caption{Copmuptational time (in seconds) required for the Gram matrix computation of the considered kernel, with different parameters.\label{fig:times}}
% \end{figure}
%
The results presented in this section suggest that the introduction of contextualized features is a promising approach, and that in principle also other kernels can benefit from such an extension.


==> ICONIP15(CameraReady)/sec_conclusions.tex <==
\section{Conclusions and future work}
In this paper, we proposed a technique to incorporate context information in the kernels that allow for an explicit feature space representation.
In particular, we defined a relationship between the explicit features where one feature can be considered as the context of another one.
We applied our idea to the $ODDK$ kernel, and slightly modified the kernel definition in order to provide an efficient algorithm for the computation of the contextualized kernel.
We evaluated the predictive performance of the resulting kernel (in two variants) over five real-world datasets, and the proposed approach shows promising results.
As future works, we plan to apply the contextualization idea to other state-of-the art graph kernels, as well as to kernels for other discrete structures.


==> ICONIP15(CameraReady)/sec_graphkernels.tex <==
\section{Definitions and notation}
Let $G=(V_G,E_G,L_G)$ be a graph, where $V_G$ is the set of vertices (or nodes), $E_G\subseteq\{(v_i,v_j) | v_i,v_j \in V_G\}$ is the set of edges and $L_G:V_G \rightarrow \Sigma$ is a labeling function mapping each vertex to an element in a fixed alphabet $\Sigma$.\\
A graph is undirected if $(i,j) \in E_G \implies (j,i)\in E_G$, otherwise it is directed.
A walk $w(u,v)$ in a graph is a sequence of nodes $v_1, \ldots,v_n$ s.t.
%$\forall_{i=1}^n v_i \in V_g$, 
 $(v_i,v_{i+1}) \in E_G$ and $v_1=u, v_n=v$.
The length of a walk $|w(u,v)|$ is defined as the number of edges in such walk.
A cycle is a walk where $v_1=v_n$. A graph is acyclic if it does not contain cycles.
A DAG is a directed acyclic graph.
A path is a walk with no repeated nodes, i.e. where $\forall_{i=1}^n \forall_{j=1}^n, i \neq j \implies v_i \neq v_j$.
A shortest path between two vertices $sp(u,v) \in V_G$ is a path with the minimum length that starts from $u$ and ends in $v$. Note that the shortest paths are not unique, but their length $|sp(u,v)|$ is.
$n\_sp(u,v)$ is a function returning the number of such shortest paths. 
%
\noindent A rooted DAG $D$ is a DAG in which one vertex $r$ has been designated as the root. The root have no incoming edges, i.e. $\not\exists u \in E_D, (u,r) \in E_D$. The function $r(D)$ returns the root of a rooted DAG.\\
A (rooted) tree is a rooted DAG where for each node there exists exactly one path connecting the root node to it. 
The children $children(v)$ of a node $v \in V_T$ in a tree are all the nodes $u \in V_T$ s.t. 
%$\exists u \in E_T, 
$(v,u) \in E_T$.
The number of children, or out-degree, of a vertex $v$ is $\rho(v)$.
Similarly we can say that $v$ is a parent
% node 
 of $u$.
% A graph is rooted if there is exactly one vertex with no parents. The function $r(G)$ returns the root node of such a graph.
$ch_i(v,G)$ is the function retuning the i-th child of $v \in V_G$ (according to a particular order).\\
% A Tree is a rooted DAG where each node has at most one parent.
% The children (or neighbors) $children(v)$ of a node $v \in V_G$ are all the nodes $u \in V_G$ s.t. $\exists u \in E_G, (v,u) \in E_G$.
% The number of children, or out-degree, of a vertex $v$ is $\rho(v)$.
% Similarly we can say that $v$ is a parent node of $u$.
% A graph is rooted if there is exactly one vertex with no parents. The function $r(G)$ returns the root node of such a graph.
% $ch_i(v,G)$ is the function retuning the i-th child of $v \in G$ (according to a particular order).\\
% A Tree is a rooted DAG where each node has at most one parent.
A proper subtree rooted at $u\in V_T$ of a tree $T$ is the subtree that comprehends $u$ and all its descendants. We will refer to it as $\subtreerootedat{u} \in T$.
%$\overset{u}{\bigtriangleup}|_{depth}$  is the subtree that comprehends $u$ and all its descendants $v$ such that the length of the shortest paths between $v$ and $u$ is at most $depth$.\\
%
We define $T_j(v,G)$ as a function returning the tree-visit of a graph $G$, rooted at $v$ and limited at height $j$. Note that this tree-visit is the shortest-path tree between $v$ and any $u \in V_G$ s.t. $|sp(u,v)|\leq j$.
%
Moreover, we denote with $T(v,G)$ the tree-visit at the maximum possible height, i.e.  $T_\infty(v,G)=T_{diam(G)}(v,G)$ where $diam(G)$ is the diameter of a graph, i.e. the length of the longest shortest path between two vertices.\\
A DAG-visit of a graph $G$, $DAG_j(v,G)$, is defined as the DAG of the shortest paths of length up to $j$. The main difference between $DAG(v,G)$ and $T(v,G)$ is that the number of nodes in the former is bounded by $|V_G|$ while in the latter it is not.
We assume the nodes in $T_j(v,G)$ or $DAG_j(v,G)$ to be ordered according to the lexicographic order between the node labels (in case two nodes have the same label, the ordering is recursively induced from the children). Such an ordering has been proven to be well-defined in~\cite{Dasan2012} for DAGs. Since trees are a special case of DAGs, the ordering relation is well-defined on trees as well.
For ease of notation, when clear from the context, the link to the graph $G$ will be omitted from the above-mentioned functions.
\section{Graph Kernels}
%
% Starting from the quantitative structure-activity relationship~\cite{King1995} assumption, the goal of a graph kernel is to express all the possible structural properties of the input graphs, or at leat the ones that are relevant for the task under consideration. 
% If we follow the graph reconstruction conjecture~\cite{Harary1964}, then the optimal kernel choice would be the all-subgraphs graph kernel~\cite{Gartner2003a}. 
% The RKHS of this kernel has a feature associated to each possible graph.
% Let us assume that an enumeration of all the possible graphs exists.
% The value of the $i^{th}$ feature for a graph $G$, $\phi_i(G)$, represents the number of subgraphs of $G$ that are isomorphic to the $i^{th}$ graph in the enumeration.
% However, this kernel also happens to be NP-complete. 
% Several efficiently computable alternatives have been proposed in literature, but efficiency comes at the cost of a reduced expressiveness.
Most of the existing graph kernels are members of the $R$-convolution kernels framework~\cite{Haussler99convolutionkernels}.
The idea of this framework is to decompose the original structure into a set of simpler structures, where a (efficient) kernel is already defined.
For example, the all-subgraphs graph kernel~\cite{Gartner2003a} has a feature associated to each possible graph. However, this kernel also happens to be NP-complete.
%In other words, with respect to the all-subgraph kernel, we are
An approach to reduce the computational complexity of the resulting kernel is to restrict the set of considered substructures of the graph. Different substructures raise different kernels. For example, in literature kernels based on random walks~\cite{Vishwanathan:uq}, shortest paths~\cite{Kriegel05shortestpath}, subtree-patterns~\cite{ShervashidzeSLMB11}, subtrees~\cite{Dasan2012} or pairs of small rooted subgraphs \cite{Costa2010} have been proposed.
The main drawback of these kernels is that they consider only local substructures of the original graphs, whose size is bounded to some limit due to computational complexity.
For this reason, in some cases they have similar predictive performances \cite{DaSanMartino2015}, probably because the different substructures can be interpreted as different, but still similar, approximations of small subgraphs of the original graph.
%
Enlarging the substructures to let the kernel consider a larger amount of information will increase the computational burden. We recall that the main challenge while designing graph kernels is the trade-off between the efficiency and the expressive power of the kernel.\\
Among the available graph kernels, the NSPDK~\cite{Costa2010} is the most related to the proposed kernel. Specifically, in the RKHS of NSPDK, every feature represents a couple of small rooted subgraphs $S_1$ and $S_2$ of a certain diameter (radius) $r$, at a certain distance, i.e. where $|sp(r(S_1),r(S_2))|=d$. In a sense, $S_1$ can be seen as a context for $S_2$ and vice versa.\\
% We compare to this kernel in our experimental assessment.
% Among the state-of-the-art kernels, 
% Indeed 
% Graph kernels are usually defined by means of simpler kernels that consider local substructures of the original graphs. Different kernels extract local features from different substructures, however, in some cases they have similar predictive performances \cite{DaSanMartino2015}, probably because the different substructures can be interpreted as different, but still similar, approximations of small subgraphs of the original graph. 
% The substructures induced by the graph kernels are usually local subgraphs whose size is bounded to some limit due to computational complexity. Enlarging the substructures to consider a wider area of shared information among different graphs will increase the computational burden. We recall that the main challenge while designing graph kernels is the trade-off between the efficiency and the expressive power of the kernel.
%
%
%
%
%\subsection{ODD kernel\label{sec:ODDkernel}}
% A DAG-visit of height $h$ rooted in node $v$ ($DAG_G^{v,h}$) is the rooted DAG where the set of vertices is defined as all the vertices reachable by a breadth-first visit in $G$ starting from $v$ and with max depth equal to $h$.
% The edge set of $DAG_G^{v,h}$ is defined as the set of all directed edges found in any shortest path between $v$ and any $u \in V_{DAG_G^{v,h}}$.
%
% By construction, a DAG-visit does not contain horizontal edges. Diamond structures allow not to replicate nodes with more than one parent.
Let us define a set of Ordered Decomposition DAGs of a graph $G$ limited to the maximum (user-specified) depth $h$ as $ODD_G=\{DAG_h(v,G) | v \in V_G\}$, where we recall that the nodes in each DAG are ordered according to a recursive relation looking at the labels of a node and all its descendants.
% Remember that, during the ODDK decomposition, several DAG-visits are generated for each node of the graph, limited to the maximum (user-specified) depth $h$:
% \[
% DDs=\{DAG_G^{v,h} | v \in V_G \}
% \]
% After an ordering step, that leads from the set of DDs to the set of Ordered DDs, or $ODDs$, 
The $ODDK$ kernel~\cite{Dasan2012} is defined as:
\[
ODDK(G_1,G_2)=\sum_{\substack{OD_1 \in ODD_{G_1}\\OD_2 \in ODD_{G_2} }} \sum_{j=1}^h \sum_{l=1}^h\sum_{\substack{v_1 \in V_{OD_1}\\v_2 \in V_{OD_2}}} C_{ST}(r(T_j(v_1)),r(T_l(v_2)))
\]
where $C_{ST}()$ is a function that defines the subtree kernel, i.e. a kernel that counts the number of shared proper subtrees between two trees.
%
This kernel allows to obtain an explicit feature space representation $\phi$~\cite{DaSanMartino2012}.
Let us define a total ordering between all the possible labeled trees that appear from the kernel application on the dataset.
Then each feature $\phi_i(G)$ represents the frequency of the $i$-th tree in the RKHS of the $ODD$ kernel.


==> ICONIP15(CameraReady)/sec_implementation.tex <==
\section{Efficient Implementation}
%ODDK features are based over DAG substructures derived from the graph. DAG-visit can have diamond structures, in which there exists nodes with more than one parent. In this case we can not define a single context for a given feature. To overcome this problem, the novel kernel bases its statistics over trees inferred by the DAG-visits. In this setting, the frequency of a feature produced by a node is based on the number of shortest path that reach the node from the root of the DAG-visit.
%\begin{definition}[Number of path towards a feature]
%We denote with $f_{path}$ the number obtained as the total number of shortest paths from the root of a DAG-visit to the nodes that has produced the feature $f$, for every DAG-visit encountered while decomposing a graph.
%\end{definition}	
%The values of $f_{path}$ is equivalent to the number of non-empty contexts of the feature $f$ encountered during the graph decomposition. Notice that, for each feature $f$, $f_{!root}$ is a lower bound of $f_{path}$. They are equal only in the case where each DAG-visit encountered during the graph decomposition is a tree. Finally, we define $freq_{tot}$ as $freq_{tot}=freq_{root}+f_{path}$. This value represent the number of times the feature $f$ appears with an associated context (possibly empty).
% \subsection{Definition of ODDWCK}
%ODDWCK exploits the graph decomposition inferred by the ODDK but it considers different statistics for the extracted features. First, given a feature, it distinguish its frequency with empty context from its frequency with non-empty context. Second, the ODDWCK statistics for features with non-empty context are based over the tree visits inferred from the DAGs. Luckily, the ODDWCK implementation does not require to explicitly build the tree visits, the statistics we need can be inferred exploiting directly the DAG-visits of the ODDK implementation. The tree visits and their associated DAG-visits differs only in case where the DAG-visits contain nodes with more than one parent. In this case, the tree visits will replicate this nodes and their associated proper subtrees. Each of the replicated nodes therefore will produce the same feature. If we count, for each node of the DAG-visit, the number of its parents we know the number of times the corresponding feature is produced. Therefore, the implementation of ODDWCK proceeds as follow: for each node of the graph a DAG-visit of a given height is generated. During the DAG-visit construction, the algorithm keeps track, for each node of the DAG-visit, the number of shortest paths from the root in a top-down fashion for free, thus for each node with more than one parent we can infer the number of times the node will be replicated, and therefore we keep track implicitly of the statistics within the tree visit. During the graph decomposition, the algorithm maintains an hashmap of the extracted ODDK features. For each of the extracted features, the algorithm keeps a record containing the frequency in which the feature has appeared with empty context and the frequency it has appeared with non-empty context within the tree visit, moreover, for each feature entry, the algorithm maintains an hashtable of its contexts. Every time a feature is generated, the algorithm proceeds to add the new feature in the context table of the features it is context of and the associated value represents the number of times the feature appears in its context.\\
%The kernel function considers the feature hashmaps of the two graphs and then it proceeds by applying the Equation \ref{Eq:ODDWCK}.
\begin{algorithm}[t]
\caption{An algorithm for computing the feature space representation of a graph $G$ according to the kernel TC with maximum (user-specified) depth $h$}\label{alg:decompose}
\begin{algorithmic}[1]
\State $\phi=\{\}$ \Comment{Implicit feature space represented as hashmap}
\ForAll{$v \in G$}
\State $D \gets DAG_{h}(v,G)$
\ForAll{$u \in$ \Call{reverseTopologicalOrder}{$D$}}
\For {$d\gets 0,\ldots,diam(D)-|sp(v,u)|$}
\If{$d=0$}
\State $f_{u,0}\gets$ $\kappa(L(u))$
\Else
\State $f_{u,d}\gets$ $\kappa(L(u) || f_{ch_1(u),d-1} || \cdots || f_{ch_{\rho(u)}(u),d-1})$
\ForAll{$ch \in children(u)$}
\State $(freq_{root},freq_{tot},{\cal C})\gets \phi_{f_{ch,d-1}}$
\If{$f_{u,d} \notin {\cal C}$}
%\State ${\cal C} \gets {\cal C}$
\State $\phi_{f_{ch,d-1}} \gets (freq_{root},freq_{tot},{\cal C} \cup {f_{u,d}})$
\EndIf
\EndFor
\EndIf
\If{$f_{u,d} \notin \phi$}
\State $\phi_{f_{u,d}}\gets (0,0,\{\})$
\EndIf 
\State $(freq_{root},freq_{tot},{\cal C})\gets \phi_{f_{u,d}}$
\If{$u = v$}
\State $freq_{root} \gets freq_{root}+1$
\EndIf
\State $\phi_{f_{u,d}} \gets (freq_{root},freq_{tot}+n\_shortest\_paths(v,u),{\cal C})$
%\EndIf
%\State $(freq_{root},freq_{tot})\gets \phi_{f}$
%\If{$u=v$} \Comment{$f$ has $\varnothing$-context}
%\State $freq_{root}\gets freq_{root}+1$
%\State $freq_{tot}\gets freq_{tot}+1$
%\EndIf
%\State $freq \gets$ \Call{getFrequency}{$u$}
%\State $freq_{tot}\gets freq_{tot}+ n\_shortest\_path(v,u)$
%\State $\phi_{f}\gets (freq_{root},freq_{tot})$
\EndFor
\EndFor
\EndFor
\State \Return the implicit feature space $\phi$ of $G$
\end{algorithmic}
\end{algorithm}
Algorithm \ref{alg:decompose} shows the pseudocode that extracts the implicit feature space $\phi$ of a graph.
%The implicit feature space 
$\phi$ is implemented as an hashmap, whose keys represent the hash of an encoded tree feature. Let us assume a perfect hash function $\kappa()$ from strings to integers is available. The entry for a feature $f$ in $\phi$ is a tuple $\phi_f=(freq_{root},freq_{tot},\mathcal{C})$, where $\mathcal{C}$ represents the set of the contexts of $f$ and it is also implemented as an hashtable.
Given a feature $f$ and a context $c \in \mathcal{C}$ s.t. $\mathcal{C} \in \phi_f$ it is possible to efficiently compute (with no additional cost when computing the tree-visits $T_j(v)$) the number of times $f$ is contained in $c$, that we will refer as $M(f,c)$. In other words, $M(f,c)$ is the number of subtrees of $c$ that are isomorphic to $f$.\\
%, that is the number of times $f$ is contained in $c$. 
%
%
%Algorithm \ref{alg:decompose} starts by initializing $\phi$ to empty. For each node $v$ of the graph $G$, we compute the DAG-visit rooted at $v$ with maximum depth $h$ (user-defined) via the ``getDAG-Visit'' function. While building the DAG-visit, we count for every node $u$ of the DAG the number of shortest paths $|SP(DAG,u)|$ ($SP$ stands for shortest paths) from the root of the DAG in a top-down fashion. Given a DAG-visit, we consider its nodes in a bottom-up fashion (thanks to the reverse topological order), in order to ensure that, for every subtree of the DAG, every child feature is extracted before its context feature. For a node of the DAG $u$, we consider all the depths of the subtree rooted at $u$, from 0 (just the root node $u$) up to the maximum depth. For each depth of the subtree rooted at $u$ we compute its corresponding ST feature. In case depth=0, then the ST feature is the hash of the label of the node, otherwise the procedure ``computeSTFeature'' computes the ST feature related to the proper subtree $\overset{u}{\bigtriangleup}|_{depth}$ (the proper subtree rooted at $u$ with depth limited to $depth$). In order to compute the composed ST feature, we consider the hashed feature of each children of $\overset{u}{\bigtriangleup}|_{depth}$ (that thanks to the reverse topological order it is guaranteed to be already computed), then we sort them and we hash the resulting encoding. The resulting (hashed )composed ST feature $c$ has to be added to the context hashmap of the features it is context of, let say $f$. The ``addContext'' procedure performs this task, by considering the hashmap $\phi$ and insert in the context map of $Contexts_f$ its context $c$ with the multiplicity $M(f,c)$ associated to it. Once we extracted the ST feature, we proceed to insert it in $\phi$. If the extracted feature $f$ is new, we initialize its entry $(freq_{root},freq_{tot})$ to $(0,0)$. If the node $u$ we are considering is the root of the current DAG-visit, it means that the feature $f$ associated to the proper subtree rooted at $u$ has no context, therefore we increment the value $freq_{root}$. We also increment $freq_{tot}$ because we are counting the total number of times the $f$ feature appears. In the case $u$ is not the root node of the DAG, we need to know how many times the subtree rooted at $u$ will appear in the different Tree-visit with different depths. This number is inferred by the function ``getFrequency''. Finally, we update the total number of times the feature $f$ appears by considering its frequency and the number of its parents.
%We ask the reader to read carefully the pseudocode in Algorithm \ref{alg:decompose} and understand the notations used; here we will focus on the more sensitive steps. 
The more sensitive steps of Algorithm~\ref{alg:decompose} are the following. Line 4 ensures that every node will be processed before its children. This allows also to compute $size(f_{u,d})$, the number of nodes in the subtree encoded by $f_{u,d}$, in a bottom-up fashion without any additional cost. In line 5, the upper limit $diam(D)-|sp(v,u)|$ is needed to consider the correct frequency of each feature when $D$ is unbalanced. In lines 7 and 9, we consider f as an hashmap indexed by the tuple $(u,d)$ that stores the values $f_{u,d}$.
%associated to the  The features $f_{u,d}$ updated in steps 7 and 9 are stored in a hashmap with keys as pairs $(u,d)$, defining the feature extracted from node $u$ with depth $d$.
The notation $||$ in line 9 refers to the concatenation operator.
%  Notice in step 24 that by incrementing $freq_{tot}$ with $n\_shortest\_paths(v,u)$ we are considering the statics implicitly inferred from the Tree-visit. Also notice that in case $u=v$, $|sp(u,v)|=1$, the path of length 0 that corresponds to the $\O$-context.
%
\begin{algorithm}[t]
\caption{An algorithm to compute the kernel function given two implicit feature spaces $\phi^1$ and $\phi^2$ of graphs $G_1$ and $G_2$}\label{alg:kf}
\begin{algorithmic}[1]
\State $score\gets 0$
\ForAll {$f_{u,d} \in \{f_{u,d} | f_{u,d} \in \phi^1 \wedge f_{u,d} \in \phi^2\}$}
\State $(freq_{root}^1,freq_{tot}^1,\mathcal{C}_{f_{u,d}}^1)\gets \phi_{f_{u,d}}^1$
\State $(freq_{root}^2,freq_{tot}^2,\mathcal{C}_{f_{u,d}}^2)\gets \phi_{f_{u,d}}^2$
\State $score\gets score + freq_{root}^{1} \cdot freq_{root}^{2} \cdot \lambda^{size(f_{u,d})}$
\ForAll{$c \in \{c | c\in \mathcal{C}_{f_{u,d}}^1 \wedge c \in \mathcal{C}_{f_{u,d}}^2\}$}
\State $(freq\_c_{root}^1,freq\_c_{tot}^1,\mathcal{C}_{c}^1)\gets \phi_{c}^1$
\State $(freq\_c_{root}^2,freq\_c_{tot}^2,\mathcal{C}_{c}^2)\gets \phi_{c}^2$
\State $score\gets score + freq\_c_{tot}^{1} \cdot freq\_c_{tot}^{2}\cdot M(f_{u,d},c)^2 \cdot \lambda^{size(f_{u,d})}$
\EndFor
\EndFor
\State \Return $score$
\end{algorithmic}
\end{algorithm}
A note on computational complexity.
Fixed as $|\phi_f|$ the number of non-zero features generated from the base kernel, the number of non-zero features $|\phi_{f \circ c}|$ of the augmented (with context information) kernel is in the worst case $|\phi_f| \cdot max_f(|\{(f,c) s.t. \phi{f \circ c} > 0 \})|$.
This implicit representation models the explicit contextualized features. The values associated to the explicit contextualized feature $f \circ \varnothing$-context ($f$ with empty context) is $freq_{root}$. Given a feature $f$ and one of its contexts $c$, the value associated to the explicit contextualized feature $f\circ c$ is given by $c_{tot} \cdot M(f,c)= c_{tot} \cdot \mathcal{C}_f[c]$.


==> ICONIP15(CameraReady)/sec_implementation_new.tex <==
\section{Efficient Implementation}
% \begin{algorithm}[t]
% \caption{An algorithm for computing the explicit feature space representation of a graph $G$ according to the kernel $TCK_{ST}$ with maximum (user-specified) height $h$ and weight factor $\lambda$}\label{alg:decomposeexpl}
% \begin{algorithmic}[1]
% \State $\phi=[0,\dots,0]$ \Comment{Explicit feature space represented as sparse vector}
% \ForAll{$v \in V_G$}
% \State $D \gets DAG_{h}(v,G)$ %line 5
% \State $f=\{\}$ \Comment{dictionary that stores the features related to a node $u$ and height $d$}
% \State $size=\{\}$ \Comment{dictionary that stores the size of each feature}
% \ForAll{$u \in$ \Call{reverseTopologicalOrder}{$D$}}
% \For {$d\gets 0,\ldots,diam(D)-|sp(v,u)|$}
% \If{$d=0$}
% \State $f_{u,0}\gets \kappa(L(u))$
% \State $size_{u,0}\gets 1$ %line 10
% \Else
% \State $(S_1,\dots,S_{\rho(u)})\gets$ \Call{sort}{$f_{ch_1(u),d-1},f_{ch_2(u),d-1},\cdots,f_{ch_{\rho(u)}(u),d-1}$}
% \State $f_{u,d}\gets \kappa(L(u) \lceil S_1 \#  S_2 \#\cdots \# S_{\rho(u)}\rfloor)$
% \State $size_{u,d}\gets 1 + \sum_{i=1}^{\rho(u)}size_{ch_i(u),d-1}$
% \ForAll{$ch \in children(u)$} %line 15
% \State $\phi_{f_{ch,d-1}\circ f_{u,d}}\gets \phi_{f_{ch,d-1}\circ f_{u,d}}+ n\_sp(v,u)\cdot \lambda^{\frac{size_{ch,d-1}}{2}}$
% \EndFor
% \EndIf
% \If{$u=v$}
% \State $\phi_{f_{u,d}\circ \varnothing}\gets \phi_{f_{u,d}\circ \varnothing} + \lambda^{\frac{size_{u,d}}{2}}$ %line 20
% \EndIf
% \EndFor
% \EndFor
% \EndFor
% \State \Return $\phi$
% \end{algorithmic}
% \end{algorithm}
% %
Algorithm \ref{alg:decomposeexpl} shows the pseudocode to decompose a graph $G$ into its explicit (sparse) feature vector $\phi$. 
%In this implementation we represent the explicit feature vector $\phi$ as a sparse vector, 
We will denote with $f$ the map that stores the keys of the local subtree features, i.e. $f_{u,d}, u \in V_G, d \in \{0,\ldots,h\}$ is the key of the subtree rooted in $u$ of height $d$. Similarly, $size$ is a map that stores the size of each feature, i.e. $size_{u,d}$ is the number of nodes that compose the feature $f_{u,d}$. Let $\kappa$ be a perfect hash function from strings to integers.
Such a function can be implemented with an incrementally-built hashmap that associates an unique id to each string. Alternatively, a normal hashing function can be used if we tolerate some clashes.  We define reserved special symbols ``$ \lceil$'', ``$\rfloor$'', ``\#'' and ``$\circ$'' that do not have to appear in the labels of the graphs and they are needed to encode subtree features into strings.
\begin{algorithm}[t]
\caption{An algorithm for computing the explicit feature space representation of a graph $G$ according to the kernel $TCK_{ST}$ with maximum (user-specified) height $h$ and weight factor $\lambda$}\label{alg:decomposeexpl}
\begin{algorithmic}[1]
\State $\phi=[0,\dots,0]$ \Comment{Explicit feature space represented as sparse vector}
\ForAll{$v \in V_G$}
\State $D \gets DAG_{h}(v,G)$ %line 5
\State $f=\{\}$ \Comment{dictionary that stores the features related to a node $u$ and height $d$}
\State $size=\{\}$ \Comment{dictionary that stores the size of each feature}
\ForAll{$u \in$ \Call{reverseTopologicalOrder}{$D$}}
\For {$d\gets 0,\ldots,diam(D)-|sp(v,u)|$}
\If{$d=0$}
\State $f_{u,0}\gets \kappa(L(u))$
\State $size_{u,0}\gets 1$ %line 10
\Else
\State $(S_1,\dots,S_{\rho(u)})\gets$ \Call{sort}{$f_{ch_1(u),d-1},f_{ch_2(u),d-1},\cdots,f_{ch_{\rho(u)}(u),d-1}$}
\State $f_{u,d}\gets \kappa(L(u) \lceil S_1 \#  S_2 \#\cdots \# S_{\rho(u)}\rfloor)$
\State $size_{u,d}\gets 1 + \sum_{i=1}^{\rho(u)}size_{ch_i(u),d-1}$
\ForAll{$ch \in children(u)$} %line 15
\State $\phi_{f_{ch,d-1}\circ f_{u,d}}\gets \phi_{f_{ch,d-1}\circ f_{u,d}}+ n\_sp(v,u)\cdot \lambda^{\frac{size_{ch,d-1}}{2}}$
\EndFor
\EndIf
\If{$u=v$}
\State $\phi_{f_{u,d}\circ \varnothing}\gets \phi_{f_{u,d}\circ \varnothing} + \lambda^{\frac{size_{u,d}}{2}}$ %line 20
\EndIf
\EndFor
\EndFor
\EndFor
\State \Return $\phi$
\end{algorithmic}
\end{algorithm}
%
 In the following, we will discuss the most sensitive steps of the algorithm. In line 6 the nodes of the DAG-visit are traversed in a reverse topological order, ensuring that every node will be processed before its parent.
%, and so the features related to the children nodes of $u$ are defined. 
In line 7, for each node $u$ of the current DAG-visit $D$, we consider all the 
heights for the feature generation. Note that when $d=0$, $f_{u,0}$ is a feature (proper subtree) of the tree $T_{|sp(v,u)|}(v)$ and when $d=diam(D)-|sp(v,u)|$, $f_{u,d}$ is a feature of $T_{diam(D)}(v)$, where $diam(D)\leq h$.
%depths up the maximum depth of the leaf of $D$. This ensure to consider all the subtrees of different depths up to the maximum possible depth.
Notice that if $D$ is unbalanced and we are considering a node $u$ whose $|sp(v,u)|$ is not maximum, then we are considering many times the feature associated to $u$ at its maximum height.
% $diam(T(u,D))$, in this way we are counting for the total number of times that feature will appear in the different tree-visits with various limited depths.
In lines 12-14, the local feature related to the current node and height is generated. The hashed feature values of the children of the current node at height $d-1$ are sorted, generating a feature of height $d$  and inducing an order on the children of every node that is the lexicographic order over the hash values of the corresponding features. This step allows us not to define any particular ordering on the nodes of $D$. Then the extracted feature is encoded and finally it is hashed.
%In lines 15-16, the algorithm generates the contextualized features by combining the local subtree features, then the entry of the contextualized feature is 
Lines 15-16 generate the contextualized features and increment their frequency in $\phi$ according to
% the weight factor $\lambda^{\frac{size_{u,d}}{2}}$ 
a weight term multiplied by $n\_sp(v,u)$. This multiplication allows us to compute the statistics related to the tree-visit while working on the smaller (in terms of number of nodes) corresponding DAG-visit. Notice that $n\_sp(v,u)$ is efficiently computed during the creation of $DAG_{h}(v,G)$ in a top-down fashion without any additional cost. 
% Finally, in case the current node $u$ is the root of $D$, then it means that the local subtrees features $f_{u,d}$ does not have any context, therefore we increment the value corresponding to the contextualized feature $\phi_{f_{u,d}\circ \varnothing}$ in line 20. 
Finally, lines 17-18 increment the value corresponding to the feature with empty context $\phi_{f_{u,d}\circ \varnothing}$. This implementation returns the explicit sparse feature vector $\phi$, therefore in order to compute the kernel function between two graphs is sufficient to compute the dot product between the two feature vectors.
%A note on computational complexity. Fixed as $|\phi_f|$ the number of non-zero features generated from the base kernel, the number of non-zero features $|\phi_{f \circ c}|$ of the augmented (with context information) kernel is in the worst case $|\phi_f| \cdot max_f(|\{(f,c) s.t. \phi_{f \circ c} > 0 \}|)$.


==> ICONIP15(CameraReady)/sec_introduction.tex <==
\section{Introduction}
In many application domains data can be naturally represented in a structured form, e.g. in Chemoinformatics~\cite{Aggarwal2010} or in natural language processing~\cite{Collins2001}.
For this reason, in the last few years an interest in machine learning techniques applicable to data represented in structured (non-vectorial) form arose \cite{Vishwanathan2010,MartinoS10}.
%
When dealing with machine learning for graph-structured data, kernel methods are one of the most popular approaches to follow. 
It just suffices to use a kernel for graphs together with any kernelized learning algorithm (e.g. SVM, SVR, KPCA, \ldots) and the user has a powerful, ready-to-use learning algorithm with strong theoretical bounds on its generalization performance.
The predictive performance of the resulting learning procedure strongly depends on the particular kernel choice.
The design of efficient graph kernels is not a trivial task, because several graph operations (e.g. the graph isomorphism)
%~\cite{JGT:JGT3190010410}
are not efficiently computable.
The idea is to design kernels that are the most expressive as possible, in order to have a small information loss.
Several alternatives have been proposed in literature. However it is difficult to state a priori which kernel will perform better in a specific task, because most of the existing kernels consider different approximations of the same local structures.
In this paper, we propose a method to enrich the feature space of a kernel with contextual information, i.e. we attach to a feature a piece of information about the topology of the graph in which that feature appeared.
We apply this idea to the ODD kernel~\cite{Dasan2012}, and we define as the context of a feature another feature from the same kernel. We give an efficient algorithm for the kernel computation, and experimentally evaluate our proposal on five real-world datasets.


==> ICONIP15(CameraReady)/section_contexts.tex <==
\section{Adding Contexts to Graph Kernels\label{sec:ODDWCK}} 
The graph kernels described in the previous section extracts local patterns of the graph as features, i.e. the feature itself does not bring any information regarding where it has appeared within the graph. The idea we propose in order to increase the expressiveness of a kernel, while preserving efficiency, is to enrich the local features (e.g. the features extracted by the $ODD$ kernel) with their contextual information. The contextual information we are interested in is a description of the topology of the graph around the extracted feature. Thus, a substructure that appears in two different graphs will match if and only if it appears within the same context in both graphs.
Considering contextual information, we obtain kernels that are more sparse.
%, and thus more discriminative than the original versions.
In some cases, the resulting kernel may be more discriminative with respect to the original one.
However, in other cases it may be too much sparse to obtain good performance. In the latter case, it can be beneficial to add the contribution of the new kernel to the original one. In our experiments, we will implement both these variants. Note that, with our proposed approach, the computation of the contributions of the contextualized kernel and of the original kernel can be performed efficiently at the same time.\\
% The idea of considering contexts to enrich the expressiveness of a kernel has been firstly introduced in the \textit{weighted decomposition kernels} family \cite{Menchetti:fk}.
% However, in this kernel we use a different idea of context, in particular every feature has a different context
% However, in this paper we consider contexts as features allows us for an efficient kernel computation.
Fixed a feature of the original graph kernel, we want the following property to hold:
$$
\sum_{c\in Contexts(f)} \phi_{f\circ c}(G) = \phi_f(G),
$$
where $\phi_f(G)$ is the frequency of a feature $f$ in the RKHS of the original kernel, and $\phi_{f \circ c}$ is the frequency of $f$ appearing within the context $c$.
% Note that $\phi_{f\circ c}$ is a feature of the new kernel that considers contexts.
From the formula it is clear that for each feature we need to consider also the empty context($\varnothing$-context), i.e. the situation in which a feature does not appear in any particular context e.g. because it has reached the maximum allowed dimension and we have no information about its context in the original graph.\\
%
%
% Finally, there is an interesting property between local features and contextualized ones we can observe. The value associated to a feature represents the number of times the substructure associated to the feature appears within the graph. A local feature will appear within a graph in different contexts. For a given substructure, if we consider all its contexts we notice that the sum of the context-based features associated to the substructure has to be equal to the value of the local feature associated to the substructure. Therefore there is a relation between the values of the contextualized features and the local ones, thus we can possibly exploit this property in order to derive the value for a local feature starting from the values of its contextualized features.\\
% Before describing in depth the contextual information over specific kernels, it is necessary to introduce the concept of empty context ($\varnothing$-context). During the graph decomposition into its features, it could happen that for a particular substructure there is no context. This can be because the extracted substructure has reached the maximum allowed dimension, or the substructure itself due to the decomposition process has no context. In this cases, the contextualized feature associated to this substructure will have an empty context.
%
In the remaining of this section, we will introduce our proposed kernel instantiating the context idea to the $ODD$ kernel.
%\subsection{Tree context kernel}
%Since we are adding contextual information from ODDK, the novel kernel we intend to define here will be called ODDK With Contexts Kernel (ODDWCK). 
%The proposed kernel is derived from the ODDK.
% % % % The proposed kernel combines the features extracted from ODDK to create new contextualized features.
% % % % A local feature is a representation of a substructure obtained during the graph decomposition.
As a feature represents a substructure, in the same way we can represent a context for a feature as a substructure of the graph, that incorporates the feature. Therefore, contexts and features can share the same representation and so it is possible that a context for a given feature can be a feature itself.
%This property allows us to exploit directly the explicit decomposition of ODD kernel: t
To compute the contextualized features we only need to combine a feature with other features representing the context in which the first feature appears in the graph.\\
%
The first important difference between the proposed Tree Context Kernel (TCK) and ODDK is that, for technical reasons, the former is defined over tree-visits while the latter over DAG-visits.
Note that the nodes of a tree-visit $T(v,G)$ of a graph $G$ can grow exponentially in its size, while if we consider a DAG-visit $DAG(v,G)$, each node in the original graph can appear at most once, thus limiting the size of the resulting structure to at most $|V_G|$ nodes.
However, in the next section we will provide an efficient implementation that does not need to store in memory the tree-visits, but only the DAG-visits.
The Tree Context Kernel can be defined as:
\begin{eqnarray}
TCK(G_1,G_2) & = & \sum_{\substack{v_1 \in V_{G_1}\\v_2 \in V_{G_2} }}\sum_{i=1}^h \sum_{j=1}^h \nonumber\\ 
%\end{eqnarray}
%\begin{eqnarray}
&  & [ \delta(T_i(v_1),T_j(v_2)) + \!\!\!\!\!\!  \sum_{\substack{\subtreerootedat{u_1} \in T_i(v_1)\\\subtreerootedat{u_2} \in T_j(v_2)}}\!\!\!\!\delta(\subtreerootedat{u_1}, \subtreerootedat{u_2})  \sum_{l=1}^{\rho(u_1)}C_{ST}(ch_l(u_1), ch_l(u_2))]\nonumber
\end{eqnarray}
\noindent where we recall that:
\[
C_{ST}(v_1,v_2)=\\
\begin{cases}
\lambda \cdot K_L(v_1,v_2) & \!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\textrm{if }v_1 \textrm{ and } v_2 \textrm{ are leaves}\\
\lambda \cdot K_L(v_1,v_2) \prod_{j=1}^{\rho(v_1)}C_{ST}(ch_j(v_1),ch_j(v_2)) & \textrm{if } \rho(v_1)=\rho(v_2) \\
0 &\text{otherwise} \\
\end{cases}
\]
and $\delta$ is the Kronecker's delta function.
We recall that $C_{ST}(v_1,v_2), v_1 \in T_1, v_2 \in T_2$ is a function that counts the common proper subtrees of two trees.
The function depends on $T_1$ and $T_2$. We decided to follow the original definition of~\cite{Collins:2001fk} omitting that dependency for ease of notation.
\\
The kernel is positive semidefinite because it is a composition of positive semidefinite kernels, defined over the ordered tree visits $T_i(v,G)=T(DAG_i(v,G))$ that are well defined as shown in~\cite{Dasan2012}.\\
Intuitively, this kernel matches two subtree features $\subtreerootedat{u_1} \in T_i(v_1,G_1), 0 \leq i \leq h$ and $\subtreerootedat{u_2} \in T_j(v_2,G_2), 0 \leq j \leq h$ in one of the following cases:
%$v_1 \in \{u \in V_ODT_{G_1}^r,h, r \in G_1\}$ and $v_2$ in one of the following cases:
\begin{itemize}
  \item both $v_1$ and $v_2$ are the root nodes of the tree visit, i.e. $u_1=v_1$ and $u_2=v_2$;
  \item $u_1$ and $u_2$ occur within the same context in both trees, i.e. their parents generate the same proper subtree.
\end{itemize}


==> sec_implementation.tex <==
\section{Efficient Implementation}
%ODDK features are based over DAG substructures derived from the graph. DAG-visit can have diamond structures, in which there exists nodes with more than one parent. In this case we can not define a single context for a given feature. To overcome this problem, the novel kernel bases its statistics over trees inferred by the DAG-visits. In this setting, the frequency of a feature produced by a node is based on the number of shortest path that reach the node from the root of the DAG-visit.
%\begin{definition}[Number of path towards a feature]
%We denote with $f_{path}$ the number obtained as the total number of shortest paths from the root of a DAG-visit to the nodes that has produced the feature $f$, for every DAG-visit encountered while decomposing a graph.
%\end{definition}	
%The values of $f_{path}$ is equivalent to the number of non-empty contexts of the feature $f$ encountered during the graph decomposition. Notice that, for each feature $f$, $f_{!root}$ is a lower bound of $f_{path}$. They are equal only in the case where each DAG-visit encountered during the graph decomposition is a tree. Finally, we define $freq_{tot}$ as $freq_{tot}=freq_{root}+f_{path}$. This value represent the number of times the feature $f$ appears with an associated context (possibly empty).
% \subsection{Definition of ODDWCK}
%ODDWCK exploits the graph decomposition inferred by the ODDK but it considers different statistics for the extracted features. First, given a feature, it distinguish its frequency with empty context from its frequency with non-empty context. Second, the ODDWCK statistics for features with non-empty context are based over the tree visits inferred from the DAGs. Luckily, the ODDWCK implementation does not require to explicitly build the tree visits, the statistics we need can be inferred exploiting directly the DAG-visits of the ODDK implementation. The tree visits and their associated DAG-visits differs only in case where the DAG-visits contain nodes with more than one parent. In this case, the tree visits will replicate this nodes and their associated proper subtrees. Each of the replicated nodes therefore will produce the same feature. If we count, for each node of the DAG-visit, the number of its parents we know the number of times the corresponding feature is produced. Therefore, the implementation of ODDWCK proceeds as follow: for each node of the graph a DAG-visit of a given height is generated. During the DAG-visit construction, the algorithm keeps track, for each node of the DAG-visit, the number of shortest paths from the root in a top-down fashion for free, thus for each node with more than one parent we can infer the number of times the node will be replicated, and therefore we keep track implicitly of the statistics within the tree visit. During the graph decomposition, the algorithm maintains an hashmap of the extracted ODDK features. For each of the extracted features, the algorithm keeps a record containing the frequency in which the feature has appeared with empty context and the frequency it has appeared with non-empty context within the tree visit, moreover, for each feature entry, the algorithm maintains an hashtable of its contexts. Every time a feature is generated, the algorithm proceeds to add the new feature in the context table of the features it is context of and the associated value represents the number of times the feature appears in its context.\\
%The kernel function considers the feature hashmaps of the two graphs and then it proceeds by applying the Equation \ref{Eq:ODDWCK}.
\begin{algorithm}[t]
\caption{An algorithm for computing the feature space representation of a graph $G$ according to the kernel TC with maximum (user-specified) depth $h$}\label{alg:decompose}
\begin{algorithmic}[1]
\State $\phi=\{\}$ \Comment{Implicit feature space represented as hashmap}
\ForAll{$v \in G$}
\State $D \gets DAG_{h}(v,G)$
\ForAll{$u \in$ \Call{reverseTopologicalOrder}{$D$}}
\For {$d\gets 0,\ldots,diam(D)-|sp(v,u)|$}
\If{$d=0$}
\State $f_{u,0}\gets$ $\kappa(L(u))$
\Else
\State $f_{u,d}\gets$ $\kappa(L(u) || f_{ch_1(u),d-1} || \cdots || f_{ch_{\rho(u)}(u),d-1})$
\ForAll{$ch \in children(u)$}
\State $(freq_{root},freq_{tot},{\cal C})\gets \phi_{f_{ch,d-1}}$
\If{$f_{u,d} \notin {\cal C}$}
%\State ${\cal C} \gets {\cal C}$
\State $\phi_{f_{ch,d-1}} \gets (freq_{root},freq_{tot},{\cal C} \cup {f_{u,d}})$
\EndIf
\EndFor
\EndIf
\If{$f_{u,d} \notin \phi$}
\State $\phi_{f_{u,d}}\gets (0,0,\{\})$
\EndIf 
\State $(freq_{root},freq_{tot},{\cal C})\gets \phi_{f_{u,d}}$
\If{$u = v$}
\State $freq_{root} \gets freq_{root}+1$
\EndIf
\State $\phi_{f_{u,d}} \gets (freq_{root},freq_{tot}+n\_shortest\_paths(v,u),{\cal C})$
%\EndIf
%\State $(freq_{root},freq_{tot})\gets \phi_{f}$
%\If{$u=v$} \Comment{$f$ has $\varnothing$-context}
%\State $freq_{root}\gets freq_{root}+1$
%\State $freq_{tot}\gets freq_{tot}+1$
%\EndIf
%\State $freq \gets$ \Call{getFrequency}{$u$}
%\State $freq_{tot}\gets freq_{tot}+ n\_shortest\_path(v,u)$
%\State $\phi_{f}\gets (freq_{root},freq_{tot})$
\EndFor
\EndFor
\EndFor
\State \Return the implicit feature space $\phi$ of $G$
\end{algorithmic}
\end{algorithm}
Algorithm \ref{alg:decompose} shows the pseudocode that extracts the implicit feature space $\phi$ of a graph.
%The implicit feature space 
$\phi$ is implemented as an hashmap, whose keys represent the hash of an encoded tree feature. Let us assume a perfect hash function $\kappa()$ from strings to integers is available. The entry for a feature $f$ in $\phi$ is a tuple $\phi_f=(freq_{root},freq_{tot},\mathcal{C})$, where $\mathcal{C}$ represents the set of the contexts of $f$ and it is also implemented as an hashtable.
Given a feature $f$ and a context $c \in \mathcal{C}$ s.t. $\mathcal{C} \in \phi_f$ it is possible to efficiently compute (with no additional cost when computing the tree-visits $T_j(v)$) the number of times $f$ is contained in $c$, that we will refer as $M(f,c)$. In other words, $M(f,c)$ is the number of subtrees of $c$ that are isomorphic to $f$.\\
%, that is the number of times $f$ is contained in $c$. 
%
%
%Algorithm \ref{alg:decompose} starts by initializing $\phi$ to empty. For each node $v$ of the graph $G$, we compute the DAG-visit rooted at $v$ with maximum depth $h$ (user-defined) via the ``getDAG-Visit'' function. While building the DAG-visit, we count for every node $u$ of the DAG the number of shortest paths $|SP(DAG,u)|$ ($SP$ stands for shortest paths) from the root of the DAG in a top-down fashion. Given a DAG-visit, we consider its nodes in a bottom-up fashion (thanks to the reverse topological order), in order to ensure that, for every subtree of the DAG, every child feature is extracted before its context feature. For a node of the DAG $u$, we consider all the depths of the subtree rooted at $u$, from 0 (just the root node $u$) up to the maximum depth. For each depth of the subtree rooted at $u$ we compute its corresponding ST feature. In case depth=0, then the ST feature is the hash of the label of the node, otherwise the procedure ``computeSTFeature'' computes the ST feature related to the proper subtree $\overset{u}{\bigtriangleup}|_{depth}$ (the proper subtree rooted at $u$ with depth limited to $depth$). In order to compute the composed ST feature, we consider the hashed feature of each children of $\overset{u}{\bigtriangleup}|_{depth}$ (that thanks to the reverse topological order it is guaranteed to be already computed), then we sort them and we hash the resulting encoding. The resulting (hashed )composed ST feature $c$ has to be added to the context hashmap of the features it is context of, let say $f$. The ``addContext'' procedure performs this task, by considering the hashmap $\phi$ and insert in the context map of $Contexts_f$ its context $c$ with the multiplicity $M(f,c)$ associated to it. Once we extracted the ST feature, we proceed to insert it in $\phi$. If the extracted feature $f$ is new, we initialize its entry $(freq_{root},freq_{tot})$ to $(0,0)$. If the node $u$ we are considering is the root of the current DAG-visit, it means that the feature $f$ associated to the proper subtree rooted at $u$ has no context, therefore we increment the value $freq_{root}$. We also increment $freq_{tot}$ because we are counting the total number of times the $f$ feature appears. In the case $u$ is not the root node of the DAG, we need to know how many times the subtree rooted at $u$ will appear in the different Tree-visit with different depths. This number is inferred by the function ``getFrequency''. Finally, we update the total number of times the feature $f$ appears by considering its frequency and the number of its parents.
%We ask the reader to read carefully the pseudocode in Algorithm \ref{alg:decompose} and understand the notations used; here we will focus on the more sensitive steps. 
The more sensitive steps of Algorithm~\ref{alg:decompose} are the following. Line 4 ensures that every node will be processed before its children. This allows also to compute $size(f_{u,d})$, the number of nodes in the subtree encoded by $f_{u,d}$, in a bottom-up fashion without any additional cost. In line 5, the upper limit $diam(D)-|sp(v,u)|$ is needed to consider the correct frequency of each feature when $D$ is unbalanced. In lines 7 and 9, we consider f as an hashmap indexed by the tuple $(u,d)$ that stores the values $f_{u,d}$.
%associated to the  The features $f_{u,d}$ updated in steps 7 and 9 are stored in a hashmap with keys as pairs $(u,d)$, defining the feature extracted from node $u$ with depth $d$.
The notation $||$ in line 9 refers to the concatenation operator.
%  Notice in step 24 that by incrementing $freq_{tot}$ with $n\_shortest\_paths(v,u)$ we are considering the statics implicitly inferred from the Tree-visit. Also notice that in case $u=v$, $|sp(u,v)|=1$, the path of length 0 that corresponds to the $\O$-context.
%
\begin{algorithm}[t]
\caption{An algorithm to compute the kernel function given two implicit feature spaces $\phi^1$ and $\phi^2$ of graphs $G_1$ and $G_2$}\label{alg:kf}
\begin{algorithmic}[1]
\State $score\gets 0$
\ForAll {$f_{u,d} \in \{f_{u,d} | f_{u,d} \in \phi^1 \wedge f_{u,d} \in \phi^2\}$}
\State $(freq_{root}^1,freq_{tot}^1,\mathcal{C}_{f_{u,d}}^1)\gets \phi_{f_{u,d}}^1$
\State $(freq_{root}^2,freq_{tot}^2,\mathcal{C}_{f_{u,d}}^2)\gets \phi_{f_{u,d}}^2$
\State $score\gets score + freq_{root}^{1} \cdot freq_{root}^{2} \cdot \lambda^{size(f_{u,d})}$
\ForAll{$c \in \{c | c\in \mathcal{C}_{f_{u,d}}^1 \wedge c \in \mathcal{C}_{f_{u,d}}^2\}$}
\State $(freq\_c_{root}^1,freq\_c_{tot}^1,\mathcal{C}_{c}^1)\gets \phi_{c}^1$
\State $(freq\_c_{root}^2,freq\_c_{tot}^2,\mathcal{C}_{c}^2)\gets \phi_{c}^2$
\State $score\gets score + freq\_c_{tot}^{1} \cdot freq\_c_{tot}^{2}\cdot M(f_{u,d},c)^2 \cdot \lambda^{size(f_{u,d})}$
\EndFor
\EndFor
\State \Return $score$
\end{algorithmic}
\end{algorithm}
A note on computational complexity.
Fixed as $|\phi_f|$ the number of non-zero features generated from the base kernel, the number of non-zero features $|\phi_{f \circ c}|$ of the augmented (with context information) kernel is in the worst case $|\phi_f| \cdot max_f(|\{(f,c) s.t. \phi{f \circ c} > 0 \})|$.
This implicit representation models the explicit contextualized features. The values associated to the explicit contextualized feature $f \circ \varnothing$-context ($f$ with empty context) is $freq_{root}$. Given a feature $f$ and one of its contexts $c$, the value associated to the explicit contextualized feature $f\circ c$ is given by $c_{tot} \cdot M(f,c)= c_{tot} \cdot \mathcal{C}_f[c]$.

